Dual Descent ALM and ADMM

Classical primal-dual algorithms attempt to solve $\max_{\mu}\min_{x} \mathcal{L}(x,\mu)$ by alternatively minimizing over the primal variable $x$ through primal descent and maximizing the dual variable $\mu$ through dual ascent. However, when $\mathcal{L}(x,\mu)$ is highly nonconvex with complex constraints in $x$, the minimization over $x$ may not achieve global optimality, and hence the dual ascent step loses its valid intuition. This observation motivates us to propose a new class of primal-dual algorithms for nonconvex constrained optimization with the key feature to reverse dual ascent to a conceptually new dual descent, in a sense, elevating the dual variable to the same status as the primal variable. Surprisingly, this new dual scheme achieves some best iteration complexities for solving nonconvex optimization problems. In particular, when the dual descent step is scaled by a fractional constant, we name it scaled dual descent (SDD), otherwise, unscaled dual descent (UDD). For nonconvex multiblock optimization with nonlinear equality constraints, we propose SDD-ADMM and show that it finds an $\epsilon$-stationary solution in $\mathcal{O}(\epsilon^{-4})$ iterations. The complexity is further improved to $\mathcal{O}(\epsilon^{-3})$ and $\mathcal{O}(\epsilon^{-2})$ under proper conditions. We also propose UDD-ALM, combining UDD with ALM, for weakly convex minimization over affine constraints. We show that UDD-ALM finds an $\epsilon$-stationary solution in $\mathcal{O}(\epsilon^{-2})$ iterations. These complexity bounds for both algorithms either achieve or improve the best-known results in the ADMM and ALM literature. Moreover, SDD-ADMM addresses a long-standing limitation of existing ADMM frameworks.

==> S2_LiteratureLong.tex <==
\section{Related Works}\label{sec: literature}
This section reviews the literature of ALM and ADMM.
\subsection{ALM}
 The asymptotic convergence and convergence rate of ALM have been extensively studied for convex programs by \cite{lanMonteiro2016alm,LiQu2019alm,LiuLiuMa2019alm,rockafellar1973multiplier,rockafellar1976augmented,xu2019iteration,xu2020first} and smooth nonlinear programs \cite{andreani2008augmented,bertsekas2014constrained}. In this subsection, we review some recent developments in ALM-based algorithms applied to nonconvex problems of the form:
\begin{align}\label{eq: alm literature}
	\min_{x\in \R^n} \left\{ F(x)~|~ h_E(x) = 0, h_I(x) \leq 0\right\}.
\end{align}
More than often, the objective $F$ is assumed to admit a composite form $f+g$, where $f$ has Lipschitz gradient and $g$ is a nonsmooth convex function.
\subsubsection{Convex Constraints}
Works \cite{hajinezhad2019perturbed,hong2016decomposing,melo2020almfullstep,melo2020iteration,sun2021algorithms,zeng2021moreau, zhang2020proximal,zhang2020global} consider affine constraints, i.e., $h_E(x) = Ax-b=0$, while inequality constraints $h_I(x)\leq 0$ are not present. For a special case with $g=0$, Hong \cite{hong2016decomposing} proposed a proximal primal-dual algorithm (prox-PDA) that finds an approximate stationary point in $\mathcal{O}(\epsilon^{-2})$ iterations, where $\epsilon>0$ measures both first-order stationarity and feasibility (``$\epsilon$-stationary point" hereafter). When $g$ is a compactly supported convex function, Hajinezhad and Hong \cite{hajinezhad2019perturbed} proposed a perturbed prox-PDA that converges to a solution with bounded infeasibility; assuming that the initial point is feasible, they established an iteration complexity of $\mathcal{O}(\epsilon^{-4})$. Zeng et al. \cite{zeng2021moreau} proposed a Moreau Envelope ALM (MEAL) for handling a general weakly convex objective function $F$, which achieves the $\mathcal{O}(\epsilon^{-2})$ iteration complexity under either the {implicit Lipschitz subgradient} condition or the {implicit bounded subgradient} condition. K. Sun and XA. Sun \cite{sun2021algorithms} proposed two variants of ALM, named LCDC-ALM and composite LCDC-ALM, for solving linearly constrained difference-of-convex (DC) programs, i.e., when $F$ is a DC function; the proposed algorithms combine ALM with a DC smoothing technique termed difference of Moreau envelopes (DME), and achieve the same $\mathcal{O}(\epsilon^{-2})$ iteration complexity.

In contrast to previously mentioned works where iteration complexities are measured by \textit{subproblem oracles}, i.e., the number of times a (proximal) augmented Lagrangian relaxation is solved, the following works study iteration complexities in terms of \textit{first-order oracles}, i.e., the number of proximal gradient steps. Under the perturbed prox-PDA framework of \cite{hajinezhad2019perturbed}, Melo et al. \cite{melo2020iteration} applied an accelerated composite gradient method (ACG) \cite{beck2009fast} to solve each proximal ALM subproblem and showed that an $\epsilon$-stationary point can be found in $\tilde{\mathcal{O}}(\epsilon^{-3})$\footnote{The notation $\tilde{\mathcal{O}}$ hides logarithmic dependence on $\epsilon^{-1}$.} ACG iterations, which can be further reduced to $\tilde{\mathcal{O}}(\epsilon^{-5/2})$ with mildly stronger assumptions. Later, Melo and Monteiro \cite{melo2020almfullstep} embedded this inner acceleration scheme in a proximal ALM with full dual multiplier update and derived an iteration complexity of $\tilde{\mathcal{O}}(\epsilon^{-3})$ ACG iterations. Zhang and Luo proposed a single-looped proximal ALM with a specially chosen proximal center; in particular, they showed that when $g$ is an indicator function of a hypercube \cite{zhang2020proximal} or a polyhedron \cite{zhang2020global}, it suffices to perform one projected gradient step in each iteration, and an $\epsilon$-stationary point can be found in $\mathcal{O}(\epsilon^{-2})$ iterations.

Works \cite{kong2020iteration,LiXu2020almv2} study the setting where convex nonlinear constraints $h_I(x)\leq 0$ are explicitly present. When $F$ is weakly convex and $h_E(x)$ is affine, Li and Xu \cite{LiXu2020almv2} combined an inexact ALM and a quadratic penalty method, and they showed that an $\epsilon$-stationary point can be found in $\tilde{\mathcal{O}}(\epsilon^{-5/2})$ adaptive accelerated proximal gradient (APG) steps. Kong et al. \cite{kong2020iteration} studied a more general setting: convex nonlinear constraints take the form $-h_I(x) \in \mathcal{K}$ where $\mathcal{K}$ is a closed convex cone. Under the same inner acceleration scheme as in \cite{melo2020almfullstep}, they showed that the proposed proximal ALM, named NL-IAPIAL, finds an $\epsilon$-stationary solution in $\tilde{\mathcal{O}}(\epsilon^{-3})$ ACG iterations.


\subsubsection{Nonconvex Constraints}
Works \cite{li2021rate,lin2019inexact, Sahin2019alm, xie2021complexity} consider nonlinear and nonconvex constraints. Sahin et al. \cite{Sahin2019alm} studied problem \eqref{eq: alm literature} with only equality constraints $h_E(x)=0$, and proposed a double-looped inexact ALM (iALM), where the augmented Lagrangian relaxation is solved by the accelerated gradient method in \cite{ghadimi2016accelerated}, and then the dual variable is updated with a small step size, which ensures that the sequence of dual variables is uniformly bounded. Assuming a technical \textit{regularity condition} that provides a convenient workaround to control primal infeasibility using dual infeasibility, the proposed iALM achieves an $\tilde{\mathcal{O}}(\epsilon^{-4})$ iteration complexity\footnote{The complexity presented in \cite{Sahin2019alm} is claimed to be wrong and corrected to $\tilde{\mathcal{O}}(\epsilon^{-4})$ by \cite{li2021rate}.}. Assuming the same regularity condition, Li et al. \cite{li2021rate} later improved the iteration complexity to $\tilde{\mathcal{O}}(\epsilon^{-3})$, which is achieved through a triple-looped iALM: each augmented Lagrangian relaxation is solved by an inexact proximal point method (iPPM), where each proximal subproblem in iPPM is further solved by an APG method. 

For problems where the aforementioned regularity condition is not satisfied, the inexact proximal point penalty (iPPP) method proposed by Lin et al. \cite{lin2019inexact} finds an $\epsilon$-stationary solution in $\tilde{\mathcal{O}}(\epsilon^{-4})$ adaptive APG steps under the requirement that the initial point is feasible. Xie and Wright \cite{xie2021complexity} 
	considered the case where the objective $F$ and constraints $h_E(x)$ are twice continuously differentiable with both Lipschitz and bounded gradient/Jacobian. They proposed a proximal ALM where each subproblem is solved by the  Newton-CG method \cite{royer2020newton}; under additional technical assumptions regarding the problem data, the proposed method finds an $\epsilon$-stationary solution in $\mathcal{O}(\epsilon^{-5.5})$ Newton-CG iterations.
	
\subsection{ADMM}\label{sec: admm lit}
The alternating direction method of multipliers (ADMM) was proposed in the mid-1970s \cite{gabay1976dual,glowinski1975approximation}, while the underlying idea has deep roots in maximal monotone operator theory \cite{eckstein1992douglas} and numerical methods for partial differential equations \cite{douglas1956numerical,peaceman1955numerical}. Commonly regarded as a variant of ALM, ADMM solves the augmented Lagrangian relaxation by alternately optimizing through blocks of variables and in this way subproblems become decoupled. Such a feature has gained ADMM considerable attentions in distributed optimization \cite{boyd2011distributed,makhdoumi_broadcast-based_2014,shi_linear_2014}. The convergence of ADMM with two block variables is proved for convex optimization problems \cite{eckstein1992douglas,gabay2024applications,gabay1976dual,glowinski1975approximation} and a convergence rate of $\mathcal{O}(1/K)$ is established \cite{he20121,he2015non,monteiro2013iteration}, where $K$ is the iteration index. See also \cite{cai2014direct,chen2016direct,chen2013convergence,davis2017three,gonccalves2016extending,han2012note,he_alternating_2012,lin2015sublinear,hong2017linear,li2015convergent,lin2015global,lin2016iteration,lin2018global} for results on convex multi-block ADMM.

In recent years, researchers have extended the ADMM framework to solve nonconvex multi-block problem \eqref{eq: mb-nlp}, where $h_i(x_i) = A_ix_i$ is affine for all $i\in [p]$ \cite{gonccalves2017convergence,hong2016convergence,jiang2019structured,lipong2015global,liu2019linearized,melo2017iteration,melo2017jacobi,wang2015convergence,wang2014convergence,wang2015global}. 
The asymptotical convergence and an iteration complexity of $\mathcal{O}(\epsilon^{-2})$ are established based on two crucial conditions on the problem data: (a) $g_p = 0$ and (b) the column space of $A_p$ contains the column space of the concatenated matrix $[A_1, \cdots, A_{p-1}]$.Condition (a) provides a way to control dual iterates by primal iterates, while condition (b) is required for ADMM to locate a feasible solution in the limit. See also \cite[Table 1]{sun2019two} for a comparison on other assumptions. These two assumptions are almost necessary for the convergence of nonconvex ADMM: when either one of the two assumptions fails to hold, divergent examples have been found. 

There are also several works investigating the convergence of nonconvex ADMM without conditions (a) and (b). In particular, Jiang et al. \cite{jiang2019structured} proposed to run ADMM on a penalty relaxation of \eqref{eq: mb-nlp} with $p+1$ blocks of variables. K. Sun and XA. Sun \cite{sun2019two,sun2021two} proposed a two-level framework that embeds a specially structured three-block ADMM inside an ALM. For weakly convex minimization with affine constraints, works \cite{zeng2021moreau,zhang2020proximal} demonstrate two multi-block variants of the proximal ALM that do not require assumptions (a) or (b).

Zhu et al. \cite{zhu2020first} considered nonlinear coupling constraints of the form $h(x_1) + Bx_2=0$. Assuming condition (a) and a straightforward extension of condition (b), i.e., the range of the nonlinear mapping $h$ belongs to the column space of the matrix $B$, the authors derived an ADMM-like algorithm named NAPP-AL, which achieves the same $\mathcal{O}(\epsilon^{-2})$ iteration complexity.

